Two Biexciton Types Coexisting in Coupled Quantum Dot Molecules

Coupled colloidal quantum dot molecules are an emerging class of nanomaterials, introducing new degrees of freedom for designing quantum dot-based technologies. The properties of multiply excited states in these materials are crucial to their performance as quantum light emitters but cannot be fully resolved by existing spectroscopic techniques. Here we study the characteristics of biexcitonic species, which represent a rich landscape of different configurations, such as segregated and localized biexciton states. To this end, we introduce an extension of Heralded Spectroscopy to resolve different biexciton species in the prototypical CdSe/CdS coupled quantum dot dimer system. We uncover the coexistence and interplay of two distinct biexciton species: A fast-decaying, strongly-interacting biexciton species, analogous to biexcitons in single quantum dots, and a long-lived, weakly-interacting species corresponding to two nearly-independent excitons separated to the two sides of the coupled quantum dot pair. The two biexciton types are consistent with numerical simulations, assigning the strongly-interacting species to two excitons localized at one side of the quantum dot molecule and the weakly-interacting species to excitons segregated to the two quantum dot molecule sides. This deeper understanding of multiply excited states in coupled quantum dot molecules can support the rational design of tunable single- or multiple-photon quantum emitters.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> xx.tex <==



==> yy.tex <==


